Telling FIBS: Probes Effectively Detect Sabotage and Catch Unverbalized Deception

Recent incidents have highlighted the challenge of monitoring LLM agents and the danger of models deceiving people. We show that white-box deception detection via probes can be scaled up to frontier monitoring settings by collecting the largest deception dataset to date for training probes and introducing a novel probe architecture which can aggregate information across many layers and tokens. Our probes surpass black-box monitors on agentic coding benchmarks, achieving 98.3% AUROC in SHADE-Arena and 98.0% in BashArena (vs. 97.7%, 97.6% resp. for action-only text monitors), and show improved efficacy as the underlying model is scaled up. We further test probes on several cases where deception cannot be determined from the context alone; in these cases of introspective deception, the ground truth can only be determined through careful elicitation or knowledge of a model's training data. In one such evaluation, we show that probes can distinguish transcripts containing a model's true hidden goal from other goals with an AUROC of up to 99.7%. Our probes also detect deception on prominent open-weight models which lie about politically sensitive topics when put under pressure. We release our training dataset, dubbed FIBS, to help drive frontier deployment of effective probes, and encourage the community to expand upon it with further examples of deception and sabotage.

==> figures/methodology/introspective_evals/twemoji_icons.tex <==
\tikzset{
  pics/twemoji robot/.style={code={
    \fill[fill={rgb,1:red,0.957;green,0.565;blue,0.047}]
      (13.5,2.625) .. controls (13.5,1.176) and (12.66,0) .. (11.625,0) .. controls (10.59,0) and (9.75,1.176) .. (9.75,2.625) .. controls (9.75,4.074) and (10.59,5.25) .. (11.625,5.25) .. controls (12.66,5.25) and (13.5,4.074) .. (13.5,2.625) -- cycle;
    \fill[fill={rgb,1:red,0.957;green,0.565;blue,0.047}]
      (-9.75,2.625) .. controls (-9.75,1.176) and (-10.59,0) .. (-11.625,0) .. controls (-12.66,0) and (-13.5,1.176) .. (-13.5,2.625) .. controls (-13.5,4.074) and (-12.66,5.25) .. (-11.625,5.25) .. controls (-10.59,5.25) and (-9.75,4.074) .. (-9.75,2.625) -- cycle;
    \fill[fill={rgb,1:red,1;green,0.675;blue,0.2}]
      (12,-0.75) .. controls (12,-1.164) and (11.664,-1.5) .. (11.25,-1.5) -- (9,-1.5) .. controls (8.586,-1.5) and (8.25,-1.164) .. (8.25,-0.75) -- (8.25,6) .. controls (8.25,6.414) and (8.586,6.75) .. (9,6.75) -- (11.25,6.75) .. controls (11.664,6.75) and (12,6.414) .. (12,6) -- cycle
      (-8.25,-0.75) .. controls (-8.25,-1.164) and (-8.586,-1.5) .. (-9,-1.5) -- (-11.25,-1.5) .. controls (-11.664,-1.5) and (-12,-1.164) .. (-12,-0.75) -- (-12,6) .. controls (-12,6.414) and (-11.664,6.75) .. (-11.25,6.75) -- (-9,6.75) .. controls (-8.586,6.75) and (-8.25,6.414) .. (-8.25,6) -- cycle;
    \fill[fill={rgb,1:red,1;green,0.8;blue,0.302}]
      (7.5,9.75) .. controls (7.5,7.68) and (4.141,6.75) .. (0,6.75) .. controls (-4.141,6.75) and (-7.5,7.68) .. (-7.5,9.75) .. controls (-7.5,11.82) and (-4.141,13.5) .. (0,13.5) .. controls (4.141,13.5) and (7.5,11.82) .. (7.5,9.75) -- cycle;
    \fill[fill={rgb,1:red,0.957;green,0.565;blue,0.047}]
      (5.25,10.438) .. controls (5.25,9.23) and (2.898,8.25) .. (0,8.25) .. controls (-2.898,8.25) and (-5.25,9.23) .. (-5.25,10.438) .. controls (-5.25,11.645) and (-2.898,12.625) .. (0,12.625) .. controls (2.898,12.625) and (5.25,11.645) .. (5.25,10.438) -- cycle;
    \fill[fill={rgb,1:red,0.133;green,0.4;blue,0.6}]
      (9,9.375) .. controls (9,8.34) and (8.16,8.25) .. (7.125,8.25) -- (-7.125,8.25) .. controls (-8.16,8.25) and (-9,8.34) .. (-9,9.375) .. controls (-9,10.41) and (-8.16,11.25) .. (-7.125,11.25) -- (7.125,11.25) .. controls (8.16,11.25) and (9,10.41) .. (9,9.375) -- cycle;
    \fill[fill={rgb,1:red,0.333;green,0.675;blue,0.933}]
      (9,9) -- (-9,9) .. controls (-9.828,9) and (-10.5,8.328) .. (-10.5,7.5) -- (-10.5,-12) -- (10.5,-12) -- (10.5,7.5) .. controls (10.5,8.328) and (9.828,9) .. (9,9) -- cycle;
    \fill[fill={rgb,1:red,0.231;green,0.533;blue,0.765}]
      (12.75,-11.25) -- (12.75,-10.5) .. controls (12.75,-9.672) and (12.078,-9) .. (11.25,-9) -- (3.055,-9) -- (0.531,-11.523) .. controls (0.238,-11.816) and (-0.238,-11.816) .. (-0.531,-11.523) -- (-3.055,-9) -- (-11.25,-9) .. controls (-12.078,-9) and (-12.75,-9.672) .. (-12.75,-10.5) -- (-12.75,-11.25) .. controls (-12.75,-12.078) and (-12.828,-12.75) .. (-12,-12.75) -- (12,-12.75) .. controls (12.828,-12.75) and (12.75,-12.078) .. (12.75,-11.25) -- cycle;
    \fill[fill={rgb,1:red,1;green,1;blue,1}]
      (8.25,2.625) .. controls (8.25,0.762) and (6.738,-0.75) .. (4.875,-0.75) .. controls (3.012,-0.75) and (1.5,0.762) .. (1.5,2.625) .. controls (1.5,4.488) and (3.012,6) .. (4.875,6) .. controls (6.738,6) and (8.25,4.488) .. (8.25,2.625) -- cycle;
    \fill[fill={rgb,1:red,0.867;green,0.18;blue,0.267}]
      (6.914,2.625) .. controls (6.914,1.496) and (6.004,0.586) .. (4.875,0.586) .. controls (3.746,0.586) and (2.836,1.496) .. (2.836,2.625) .. controls (2.836,3.754) and (3.746,4.664) .. (4.875,4.664) .. controls (6.004,4.664) and (6.914,3.754) .. (6.914,2.625) -- cycle;
    \fill[fill={rgb,1:red,1;green,1;blue,1}]
      (-1.5,2.625) .. controls (-1.5,0.762) and (-3.012,-0.75) .. (-4.875,-0.75) .. controls (-6.738,-0.75) and (-8.25,0.762) .. (-8.25,2.625) .. controls (-8.25,4.488) and (-6.738,6) .. (-4.875,6) .. controls (-3.012,6) and (-1.5,4.488) .. (-1.5,2.625) -- cycle;
    \fill[fill={rgb,1:red,0.961;green,0.973;blue,0.98}]
      (8.25,-5.625) .. controls (8.25,-6.66) and (7.41,-7.5) .. (6.375,-7.5) -- (-6.375,-7.5) .. controls (-7.41,-7.5) and (-8.25,-6.66) .. (-8.25,-5.625) .. controls (-8.25,-4.59) and (-7.41,-3.75) .. (-6.375,-3.75) -- (6.375,-3.75) .. controls (7.41,-3.75) and (8.25,-4.59) .. (8.25,-5.625) -- cycle;
    \fill[fill={rgb,1:red,0.8;green,0.839;blue,0.867}]
      (-0.75,-3.75) -- (0.75,-3.75) -- (0.75,-7.5) -- (-0.75,-7.5) -- cycle
      (-4.5,-3.75) -- (-3,-3.75) -- (-3,-7.5) -- (-4.5,-7.5) -- cycle
      (3,-3.75) -- (4.5,-3.75) -- (4.5,-7.5) -- (3,-7.5) -- cycle
      (-8.25,-5.625) .. controls (-8.25,-6.531) and (-7.605,-7.289) .. (-6.75,-7.461) -- (-6.75,-3.789) .. controls (-7.605,-3.961) and (-8.25,-4.719) .. (-8.25,-5.625) -- cycle
      (6.75,-3.789) -- (6.75,-7.461) .. controls (7.605,-7.289) and (8.25,-6.531) .. (8.25,-5.625) .. controls (8.25,-4.715) and (7.605,-3.961) .. (6.75,-3.789) -- cycle;
    \fill[fill={rgb,1:red,0.867;green,0.18;blue,0.267}]
      (-2.836,2.625) .. controls (-2.836,1.496) and (-3.746,0.586) .. (-4.875,0.586) .. controls (-6.004,0.586) and (-6.914,1.496) .. (-6.914,2.625) .. controls (-6.914,3.754) and (-6.004,4.664) .. (-4.875,4.664) .. controls (-3.746,4.664) and (-2.836,3.754) .. (-2.836,2.625) -- cycle;}},
}

